Beyond Distribution Shift: Spurious Features Through the Lens of Training Dynamics

Deep Neural Networks (DNNs) are prone to learning spurious features that correlate with the label during training but are irrelevant to the learning problem. This hurts model generalization and poses problems when deploying them in safety-critical applications. This paper aims to better understand the effects of spurious features through the lens of the learning dynamics of the internal neurons during the training process. We make the following observations: (1) While previous works highlight the harmful effects of spurious features on the generalization ability of DNNs, we emphasize that not all spurious features are harmful. Spurious features can be "benign" or "harmful" depending on whether they are "harder" or "easier" to learn than the core features for a given model. This definition is model and dataset-dependent. (2) We build upon this premise and use instance difficulty methods (like Prediction Depth (Baldock et al., 2021)) to quantify "easiness" for a given model and to identify this behavior during the training phase. (3) We empirically show that the harmful spurious features can be detected by observing the learning dynamics of the DNN's early layers. In other words, easy features learned by the initial layers of a DNN early during the training can (potentially) hurt model generalization. We verify our claims on medical and vision datasets, both simulated and real, and justify the empirical success of our hypothesis by showing the theoretical connections between Prediction Depth and information-theoretic concepts like V-usable information (Ethayarajh et al., 2021). Lastly, our experiments show that monitoring only accuracy during training (as is common in machine learning pipelines) is insufficient to detect spurious features. We, therefore, highlight the need for monitoring early training dynamics using suitable instance difficulty metrics.

==> sections/old_v1/abstract.tex <==
Deep Neural Networks (DNNs) are prone to learning \emph{shortcut} patterns that damage the generalization of the DNN during deployment. This paper aims to better understand shortcut learning through the lens of the learning dynamics of the internal neurons during the training process. We make the following observations: (1) While previous works treat shortcuts as synonymous with spurious correlations, we emphasize that not all spurious correlations are shortcuts. We show that shortcuts are only those spurious features that are ``easier'' than the core features. (2) We build upon this premise and use \emph{instance difficulty} methods (like Prediction Depth~\citep{baldock2021_predictionDepth}) to quantify ``easy'' and to identify this behavior during the training phase. (3) We empirically show that shortcut learning can be detected by observing the learning dynamics of the DNN's \emph{early layers}. In other words, easy features learned by the initial layers of a DNN early during the training are potential shortcuts. We verify our claims on medical and vision datasets, both simulated and real, and justify the empirical success of our hypothesis by showing the theoretical connections between Prediction Depth and information-theoretic concepts like $\mathcal{V}$-usable information~\citep{swabha_pvi}. Lastly, our experiments show the insufficiency of monitoring only accuracy plots during training (as is common in machine learning pipelines). We highlight the need for monitoring early training dynamics using example difficulty metrics.

==> sections/old_v1/background.tex <==
 In this section, we formalize the notion of spurious features, shortcuts, and task difficulty. Let $P_{tr}$ and $P_{te}$ be the training and test distributions defined over the random variables $\rmX$ (input), $\rvy$ (label), and $\rvs$ (\emph{latent} spurious feature).


\paragraph{Definition-1 (Spurious Feature $\rvs$):} A latent feature $\rvs$ is called spurious if it is correlated with label $\rvy$ in the training data but not in the test data. Specifically, the joint probability distributions $P_{tr}$ and $P_{te}$ can be factorized as follows.
\begin{equation}
    P_{tr}(\rmX,\rvy,\rvs) = P_{tr}(\rmX|\rvs,\rvy) P_{tr}(\rvs|\rvy)P_{tr}(\rvy) \nonumber
\end{equation}
\begin{equation}
    P_{te}(\rmX,\rvy,\rvs) = P_{tr}(\rmX|\rvs,\rvy) P_{te}(\rvs)P_{tr}(\rvy). \nonumber
\end{equation}
The variable $\rvs$ appears to be causally related to $\rvy$ but is not. This is shown in Fig-\ref{fig:spurious_vs_shortcut}. We also need a notion of task difficulty. The difficulty of a task depends on the model and data distribution ($\rmX, \rvy$).



\paragraph{Definition-2 (Task Difficulty $\Psi$):}
Let $\Psi^{P}_{\mathcal{M}}(\rmX \rightarrow \rvy)$ indicates the difficulty of predicting $\rmX \rightarrow \rvy$ for a model $\mathcal{M}$, where $\rmX,\rvy \sim P$. Consider a joint distribution $(\rmX,\rvy,\rvt) \sim P$ for two tasks, $\rvt$, and $\rvy$. Then, $\Psi^{P}_{\mathcal{M}}(\rmX \rightarrow \rvy) > \Psi^{P}_{\mathcal{M}}(\rmX \rightarrow \rvt)$ indicates that the task $\rmX \rightarrow \rvy$ is harder than $\rmX \rightarrow \rvt$ for a given model $\mathcal{M}$.


\paragraph{Definition-3 (Shortcut):} The spurious feature $\rvs$ is a potential shortcut for model $\mathcal{M}$ iff $\Psi^{P_{tr}}_{\mathcal{M}}(\rmX \rightarrow \rvy) > \Psi^{P_{tr}}_{\mathcal{M}}(\rmX \rightarrow \rvs)$. In other words, given the input $\rmX$, predicting spurious feature $\rvs$ is easier for $\mathcal{M}$ than predicting the true label $\rvy$.

The definitions make it clear that “shortcut” is not just related to the dataset alone but is also closely tied to the model and the task. What is a shortcut for one model may not be so for another. E.g., consider input  $X = \{x_1,x_2,…,x_n\}$ that can be viewed as both a vector or a set. Consider two models, $f_1$, which is a permutation-invariant function (like Deep Sets~\citep{deep_sets}), and $f_2$ is a coordinate-sensitive function (e.g., MLP). If the spurious feature is always in $x_1$, it can be a shortcut for $f_2$, but may not be so for $f_1$ because $f_1$ is coordinate agnostic. In fact one can show~\citep{deep_sets} that $f_1 = \rho(\sum_i \phi(x_i))$  for suitable transformations $\phi$ and $\rho$.

% Note that we use the term ``potential shortcut'' because, in the presence of multiple spurious features, \citet{scimeca2021shortcut} empirically show that the model selectively favors the easiest spurious feature.


We now explain two metrics (Prediction Depth and $\mathcal{V}$-Usable Information) to measure $\Psi^{P}_{\mathcal{M}}$. \citet{baldock2021_predictionDepth} proposed the notion of Prediction Depth (PD) to estimate example difficulty. The PD of input is defined as the minimum number of layers required by the model to classify the input. Our work relies on monitoring early training dynamics using example difficulty metrics, and we use PD estimation for this purpose. The PD metric is also well-suited for our work as it is defined for easy inputs even when the DNN is not fully trained. We use a binary classification setting to explain the concepts used in this section. 

\paragraph{Notion of Prediction Depth:} The PD is defined by building $k$-NN classifiers on the embedding layers of the model. The PD is simply the earliest layer after which all subsequent $k$-NN predictions remain the same (0 or 1):
\begin{equation}
    \text{PD} = \min \argmax_{n} \left[ \prod_{i=n}^{N}f_{knn}(\phi^i) + \prod_{i=n}^{N}(1-f_{knn}(\phi^i)) \right], \nonumber
\end{equation}

$f_{knn}$ is a $k$-NN classifier that outputs 0 or 1 based on a given threshold (see Appendix-\ref{appdx:undefined_PD} for details), $\phi^i$ is the feature embedding for the given input at layer-$i$, and $N$ is the index of the final layer of the model. The lower the PD of input, the easier it is to classify. We also use the notion of undefined PD to work with models that are not fully trained. We treat $k$-NN predictions close to 0.5 (for a binary classification setting) as invalid. If the $k$-NN predictions for the last three layers (for a given input to the model) are invalid, we treat the PD of the input as undefined (see Appendix-\ref{appdx:undefined_PD}). Figure-\ref{fig:pd_plot_explain} illustrates how to read the PD plots used in our experiment.

 \begin{figure*}[ht!]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth, trim = 0cm 6cm 0cm 0cm]{figures/pd_plot_explain.pdf}}
    \caption{Examples of PD plots (for DenseNet-121) at different stages of the training process. The red bar indicates samples with undefined PD, and the dotted vertical line indicates the mean PD of the plot. Notice that the undefined samples (shown in red) slowly accumulate in layer 88 as training progresses. This is because the model needs more time to learn the challenging samples which accumulate at higher prediction depth, i.e., later layers.}
    \label{fig:pd_plot_explain}
\end{figure*}
%  trim=left bottom right top

\paragraph{Notion of $\mathcal{V}$-Usable Information:} The Mutual Information between input and output, $I(X; Y)$, is invariant with respect to lossless encryption of the input, i.e., $I(\tau(X); Y) = I(X; Y)$. Such a definition assumes unbounded computation and is counter-intuitive to define task difficulty as heavy encryption of $X$ does not change the task difficulty. The notion of \textit{``Usable Information''} introduced by~\citet{xu2020_usable_info} assumes bounded computation based on the model family $\mathcal{V}$ under consideration. Usable information is measured under a framework called \textit{predictive $\mathcal{V}$-information}~\citep{xu2020_usable_info}. \citet{swabha_pvi} introduce \textit{pointwise $\mathcal{V}$-information} (PVI) for measuring example difficulty. 
\begin{align} \label{pvi_eq}
    \text{PVI}(x \rightarrow y) = -\log_2g[\phi](y) + \log_2g'[x](y), \\
    \text{s.t.}  \quad g,g' \in \mathcal{V} \nonumber
\end{align}
The function $g$ is trained on $(\phi,y)$ input-label pairs, where $\phi$ is a null input that provides no information about the label $y$. $g'$ is trained on $(x,y)$ pairs from the training data. Lower PVI instances are harder for $\mathcal{V}$ and vice-versa. Since the first term in Eq-\ref{pvi_eq} corresponding to $g$ is independent of the input $x$, we only consider the second term having $g'$ in our experiments. In what follows, we relate the notions of PD and $\mathcal{V}$-usable information. We use $\mathcal{V}_{cnn}$ (of finite depth and width) in our proof as our experiments mainly use CNN architectures. 
\paragraph{Proposition 1:} (Informal) Consider two datasets: $D_s \sim P_{tr}(\rmX,\rvy)$ with spurious features and $D_i \sim P_{te}(\rmX,\rvy)$ without them. For some mild assumptions on PD (see Appendix-\ref{subsec:proof_prop1}), if the mean PD of $D_s$ is less than the mean PD of $D_i$, then the $\cV_{cnn}$-usable-information for $D_s$ is larger than the  $\cV_{cnn}$-usable-information for $D_i$: $\cI_{\cV_{cnn}}^{D_s}(X \rightarrow Y) > \cI_{\cV_{cnn}}^{D_i}(X \rightarrow Y)$. \\

See proof in Appendix-\ref{subsec:proof_prop1}. The proposition intuitively implies that a sufficient gap between the mean PD of spurious and core features can result in spurious features having more $\cV_{cnn}$-usable information than core features. In such a scenario, the model will be more inclined to learn spurious features instead of core ones. This proposition justifies using the PD metric to detect shortcut learning, as demonstrated in the following experiments.

==> sections/old_v1/experiments.tex <==
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-1.0ex]{0pt}{0pt}}   % = `bottom' strut

We set up four experiments to evaluate our hypothesis. 
\textit{First}, we consider two kinds of datasets, one where the spurious feature is easier than the core feature and another where the spurious feature is harder. We train a classifier on each dataset and observe that the model can learn the easy spurious feature but not the harder one. This experiment demonstrates that not all spurious correlations are shortcuts, but only those spurious features that are easier than the core features are potential shortcuts.
\textit{Second}, we use medical and vision datasets to demonstrate how monitoring the learning dynamics of the initial layers can reveal suspicious shortcut learning activity. We show that an early peak in the PD plot indicates potential shortcuts, and visualization techniques like grad-CAM can provide intuition about the feature used at that layer.
\textit{Third}, we show how shortcuts can often be detected relatively early during training. This is because initial layers which learn the shortcuts converge very early during the training. We observe this by monitoring PD plots across training epochs. In all of our experiments, the shortcut is revealed by the PD plot within two epochs of training.
\textit{Fourth}, we show that datasets with easy spurious features have more ``usable information''~\citep{swabha_pvi} compared to their counterparts without such features. Due to higher usable information, the model requires fewer layers to classify the images with spurious features. We use this experiment to empirically justify Proposition-1 outlined in Appendix-\ref{subsec:proof_prop1}.

\setcounter{figure}{3} 
\setcounter{table}{1} 
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.0\textwidth, trim = 0cm 8cm 0cm 0cm]{figures/domino_fig.pdf}    \label{fig:domino_fig}
\end{figure*}
%  trim=left bottom right top

\subsection{Not all spurious correlations are shortcuts}
\label{subsec:not_all_spurious}
We use the Dominoes binary classification dataset (formed by concatenating two datasets vertically; see Fig-3) similar to the setup of \citet{kirichenko2022_last_layer_retraining}. The bottom (top) image acts as the core (spurious) feature. Images are of size $64 \times 32$. We construct three pairs of domino datasets such that each pair has both a hard and an easy spurious feature with respect to the common core feature (see Table-1). We use classes \{0,1\} for MNIST and SVHN, \{coat,dress\} for FMNIST,  and \{airplane, automobile\} for CIFAR10. We also include two classes from Kuzushiji-MNIST (or KMNIST) and construct a modification of this dataset called KMNpatch, which has a spurious patch feature (5x5 white patch on the top-left corner) for one of the two classes of KMNIST. The spurious features are perfectly correlated with the target. The order of dataset difficulty based on the mean-PD is as follows: KMNpatch(1.1) $<$ MNIST(2.2) $<$ FMNIST(3.9) $<$ KMNIST(5) $<$ SVHN(5.9) $<$ CIFAR10(6.8). We use a ResNet18 model and measure the test and core-only accuracies. The test accuracy is measured on a held-out dataset sampled from the same distribution. For the core-only accuracy, we blank out the spurious feature (top-half image) by replacing it with zeroes (same as~\citet{kirichenko2022_last_layer_retraining}). The higher the core-only accuracy, the lesser the model's reliance on the spurious feature.


% \begin{minipage}{0.4\textwidth}  %------------------for Figure-------------
% \begin{figure}[H]
% \centering
% \includegraphics[width=1\textwidth]{figures/domino_pic.pdf}
% \caption{{\color{magenta}Dominoes Dataset}}\label{fig:domino_pic_label}
% \end{figure}
% \end{minipage}
% \begin{minipage}[HT]{0.6\textwidth}      %------------------for Table-------------
% % \centering
% \begin{table}[H]
% \centering
% %\captionsetup{type=table} %% tell latex to change to table
%     \tiny
%     \begin{tabular}{cccc}
%         \hline 
%         \multicolumn{1}{c}{\bf Dataset}  &\multicolumn{1}{c}{\bf Is spurious} &\multicolumn{1}{c}{\bf Test} &\multicolumn{1}{c}{\bf Core-only} \Tstrut{}\\ 
%         \multicolumn{1}{c}{\bf (Spurious-Core)} &\multicolumn{1}{c}{\bf harder than core?} &\multicolumn{1}{c}{\bf Accuracy} &\multicolumn{1}{c}{\bf Accuracy} \Bstrut{}\\ 
%         \hline 
%         CIF(6.8) - FMN(3.9) & yes & 99.12$\pm$0.27\% & 98.95$\pm$0.30\% \Tstrut{}\\
%         MN(2.2) - FMN(3.9) & no & 99.95$\pm$0.05\% & 50.75$\pm$2.96\% \Bstrut{}\\
%         \hline
%         CIF(6.8) - KMN(5) & yes & 98.91$\pm$0.16\% & 98.30$\pm$1.08\% \Tstrut{}\\
%         MN(2.2) - KMN(5) & no & 99.97$\pm$0.05\% & 50.48$\pm$2.64\% \Bstrut{}\\
%         \hline
%         CIF(6.8) - MN(2.2) & yes & 99.74$\pm$0.07\% & 99.5$\pm$0.66\% \Tstrut{}\\
%         KMNpatch(1.1) - MN(2.2) & no & 99.97$\pm$0.04\% & 68.78$\pm$20.03\% \Bstrut{}\\
%         \hline 
%     \end{tabular}
% \caption{{\color{magenta}Results for the Dominoes experiment averaged across 4-runs. Numbers in bracket show mean-PD (dataset-difficulty). Core-only accuracy indicates the model's reliance on core features. Models achieve high core-only accuracy when spurious features are harder than core features.}}\label{dominoes_expts}
% \end{table}
% \end{minipage} 

Table 1 shows that all datasets achieve a high test accuracy as expected. The core-only accuracy stays high ($>$98\%) for datasets where the spurious feature is harder to learn than the core feature, indicating the model's high reliance on core features. When the spurious feature is easier than the core, the model learns to leverage them, and hence the core-only accuracy drops to nearly random chance ($\sim$50\%). Interestingly, the KMNpatch-MN results have a much higher core-only accuracy ($\sim$69\%) and a more significant standard deviation. We explain this phenomenon in Appendix-\ref{appdx:pd_perspective_feature_learning}. This experiment demonstrates that a spurious feature that is harder than the core feature fails to act as a shortcut that the model can leverage to ``cheat''.

\subsection{Monitoring Initial Layers Can Reveal Suspicious Shortcut Learning Activity}
%  Initial layers hold valuable information about shortcuts!
\label{subsec:main_expts_toy_medical}

\paragraph{Synthetic Shortcut on Toy Dataset:} To provide a proof of concept, we demonstrate our method on the Kuzushiji-MNIST (KMNIST)~\citep{kmnist} dataset comprising Japanese Hiragana characters. The dataset has ten classes and images of size $28\times28$, similar to MNIST. We insert a white patch (spurious feature) at a particular location for each of the ten classes. The location of the patch is class-specific. We train two VGG16 models, one on the KMNIST with a patch shortcut ($\mathcal{M}_{sh}$) and another on the original KMNIST without the patch ($\mathcal{M}_{orig}$). 

\begin{figure*}[!t]
    \centering
    \centerline{\includegraphics[width=1\textwidth, trim = 0cm 2cm 0cm 0cm]{figures/kmnist_expts.pdf}}
    \caption{Top row shows three reference datasets and their corresponding prediction depth (PD) plots. The datasets are ordered based on their difficulty (measured using mean PD shown by dotted vertical lines): KMN w/ sh.(1.1) $<$ MNIST(2.2) $<$ FMNIST(3.9) $<$ KMN w/o sh.(5) $<$ SVHN(5.9) $<$ CIFAR10(6.8). The bottom row shows the effect of the shortcut on the KMNIST dataset. The yellow region on the axis indicates the expected difficulty of classifying KMNIST. While the original KMNIST lies in the yellow region, the shortcut significantly reduces the task difficulty. The Grad-CAM shows that the model focuses on the spurious patch.}
    \label{fig:kmnist_expts}
\end{figure*}
%  trim=left bottom right top

Fig-\ref{fig:kmnist_expts} shows the prediction depth (PD) plots for this experiment. The vertical dashed lines show the mean PD for each plot. Fig-\ref{fig:kmnist_expts}D shows that KMNIST with patch has a much lower mean PD than all the other datasets, and the PD plot is also highly skewed towards the initial layers. This suspicious behavior is because the white patch is a very easy feature, and hence the model only needs a single layer to detect it. The Grad-CAM maps for layer-1 confirm this by showing that $\mathcal{M}_{sh}$ focuses mainly on the patch (see Fig-\ref{fig:kmnist_expts}D), and hence the test accuracy on the original KMNIST images is very low ($\sim$8\%). The PD plot for $\mathcal{M}_{orig}$ (see Fig-\ref{fig:kmnist_expts}E) is not as skewed toward lower depth as the plot for $\mathcal{M}_{sh}$. This is expected as $\mathcal{M}_{orig}$ is not looking at the spurious patch and therefore utilizes more layers to make the prediction. The mean PD for $\mathcal{M}_{orig}$ suggests that the original KMNIST is harder than Fashion-MNIST but easier than CIFAR10. $\mathcal{M}_{orig}$ also achieves a higher test accuracy ($\sim$98\%). 

This experiment demonstrates how models that learn spurious features ($\mathcal{M}_{sh}$) exhibit PD plots that are suspiciously skewed towards the initial layers. The skewed PD plot should raise concerns, and visualization techniques like Grad-CAM can aid our intuition about what spurious feature the model may be utilizing at any given layer. 

\paragraph{Semi-Synthetic Shortcut on Medical Datasets:} \label{sec:semi_synth_expts} We follow the procedure by \citet{degrave_covid_shortcut} to create the ChestX-ray14/GitHub-COVID dataset. This dataset comprises Covid19 positive images from Github Covid repositories and negative images from ChestX-ray14 dataset~\citep{wang_chestxray14_dataset}. In addition, we also create the Chex-MIMIC dataset following the procedure by \citet{puli2021_nurd}. This dataset comprises 90\% images of Pneumonia from Chexpert~\citep{chexpert_dataset} and 90\% healthy images from MIMIC-CXR~\citep{mimic_cxr_dataset}. We train two DenseNet121 models,  $\mathcal{M}_{covid}$ on the ChestX-ray14/GitHub-COVID dataset, and $\mathcal{M}_{chex}$ on the Chex-MIMIC dataset. We use DenseNet121, a common and standard architecture for medical image analysis. Images are resized to $512\times512$. 

\begin{figure}[htbp!]
    \centering
    \centerline{\includegraphics[width=0.85\textwidth, trim = 0cm 6cm 0cm 0cm]{figures/semi_synthetic_medical_shortcut.pdf}}
    \caption{PD plots for two DenseNet-121 models trained on Chex-MIMIC and ChestX-ray14/GitHub-COVID datasets are shown in the figure, along with their corresponding Grad-CAM visualizations. Both PD plots exhibit a very high peak in the initial layers (1 to 4), indicating that the models use very easy features to make the predictions.
    }
    \label{fig:semi_synthetic_medical_shortcut}
\end{figure}
%  trim=left bottom right top

Fig-\ref{fig:semi_synthetic_medical_shortcut} shows the PD plots for $\mathcal{M}_{chex}$ and $\mathcal{M}_{covid}$. Both the plots are highly skewed towards initial layers, similar to the KMNIST with patch shortcut in Fig-\ref{fig:kmnist_expts}D. This again indicates that the models are using very easy features to make the predictions, which is concerning as the two tasks (pneumonia and covid19 detection) are hard tasks even for humans. Examining the Grad-CAM maps at layer-4 reveals that these models focus on spurious features outside the lung region, which are irrelevant because both diseases are known to affect mainly the lungs. The reason for this suspicious behavior is that, in both these datasets, the healthy and diseased samples have been acquired from two different sources.
This creates a spurious feature because source-specific attributes or tokens are predictive of the disease and can be easily learned, as pointed out by \citet{degrave_covid_shortcut}.


\paragraph{Real Shortcut on Medical Dataset:} For this experiment, we use the NIH dataset~\citep{nih_dataset} which has the popular chest drain spurious feature (for Pneumothorax detection)~\citep{luke_tube_in_lung}. Chest drains are used to treat positive Pneumothorax cases. Therefore, the presence of a chest drain in the lung is positively correlated with the presence of Pneumothorax and can be used by the deep learning model~\citep{luke_tube_in_lung}. Appendix-\ref{subsec:nih_chest_drains} outlines the procedure we use to obtain chest drain annotations for the NIH dataset. We train a DenseNet121 model ($\mathcal{M}_{nih}$) for Pneumothorax detection on NIH images of size $128\times128$. 

\begin{figure*}[h!]
    \centering
    \centerline{\includegraphics[width=0.9\textwidth, trim = 0cm 7cm 3cm 0cm]{figures/nih_results2.pdf}}
    \caption{Shortcut learning on NIH dataset. (A) PD plot for DenseNet-121 trained on NIH shows prominent peaks in the initial layers. (B, C) Grad-CAM reveals that the initial layers use irrelevant artifacts and chest drains as shortcuts for classification. (D) The chest drain spurious feature affects the AUC performance of the model. The X-axis (Y-axis) shows the false positive (true positive) rate.}
    \label{fig:nih_results}
\end{figure*}
%  trim=left bottom right top

Fig-\ref{fig:nih_results}A shows the PD plot for $\mathcal{M}_{nih}$. We observe that the distribution is not as skewed as the plots in the previous experiments. This is because all the images come from a single dataset (NIH). However, we do see suspicious peaks at the initial layers. Pneumothorax classification is challenging even for radiologists; hence, peaks at the initial layers raise suspicion. The Grad-CAM maps in Figs-\ref{fig:nih_results}B \& \ref{fig:nih_results}C reveal that the initial layers look at irrelevant artifacts and chest drains in the image. This provides evidence for shortcut learning happening in the initial layers. Fig-\ref{fig:nih_results}D shows that the AUC performance is 0.94 when the diseased patients have a chest drain and 0.74 when they don't. In both cases, the set of healthy patients remains the same. This observation is consistent with the findings of \citet{luke_tube_in_lung} and indicates that the model looks at chest drains to classify positive Pneumothorax cases. 

The above experiments demonstrate how a peak located in the initial layers of the PD plot should raise suspicion, especially when the classification task is challenging. Visualization techniques like Grad-CAM can further aid our intuition and help identify the shortcuts being learned by the model. This approach works well even for realistic scenarios and challenging spurious features (like chest drain for Pneumothorax classification), as shown above. Appendix-\ref{appdx:vision_expts} includes additional results on vision datasets.

\subsection{Detecting Shortcuts Early}
\label{expt:detect_shortcut_early}

Fig-\ref{fig:pd_evolution_nih} shows the evolution of the PD plot across epochs for $\mathcal{M}_{nih}$ (which is the model used in Fig-\ref{fig:nih_results}). This visualization helps us observe the training dynamics of the various layers. The red bar in the PD plots shows the samples with undefined prediction depths. 

\begin{figure*}[t!]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth, trim = 0cm 4cm 0cm 0cm]{figures/nih_evolution_pd_plots.pdf}}
    \caption{Evolution of PD plot across epochs shows the training dynamics of the DNN on the NIH dataset. The initial peaks (layers-4\&40) are relatively stable throughout training, whereas the later peaks (layer-88) change with time. The initial layers learn the easy shortcuts, which can be detected early during the training. Samples with undefined PD (shown in red) take more time to converge and eventually accumulate in the later layers (layer 88 in this case).}
    \label{fig:pd_evolution_nih}
\end{figure*}
%  trim=left bottom right top

These plots reveal several useful insights into the learning dynamics of the model. Firstly, we see three prominent peaks in epoch-1 at layers-4,40,88 (see Fig-\ref{fig:pd_evolution_nih}A). The magnitude of the initial peaks (like layers-4\&40) remains nearly constant throughout the training. These peaks correspond to shortcuts, as discussed in the previous section. This indicates that easy shortcuts can often be identified early (epoch-1 in this case). Fig-\ref{fig:epoch_2_pd_plot} shows the PD plots at epoch-2 for other datasets with shortcuts. It is clear from Fig-\ref{fig:epoch_2_pd_plot} that the suspiciously high peak at the initial layer is visible in the \textit{second epoch} itself. The Grad-CAM maps reveal that this layer looks at irrelevant artifacts in the dataset. This behavior is seen in all datasets shown in Fig-\ref{fig:epoch_2_pd_plot}. 

\begin{figure*}[h!]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth, trim = 0cm 9cm 0cm 0cm]{figures/epoch_2_pd_plot.pdf}}
    \caption{Epoch-2 PD plots for various datasets with shortcuts. The high spurious peak in the initial layer is visible in all the datasets indicating that shortcuts can be detected early during the training.}
    \label{fig:epoch_2_pd_plot}
\end{figure*}
%  trim=left bottom right top

Secondly, we also see that accuracy or AUC plots do not reveal shortcut learning patterns. We need to monitor the training dynamics using suitable metrics (like PD) to detect this behavior. Thirdly, the red peak (undefined samples) decreases in magnitude with time, and we see a proportional increase in the layer-88 peak. This corroborates well with the observation that later layers take more time to converge~\citep{rahaman2019spectral,mangalam2019deep,zeiler2014visualizing}. Therefore, samples with higher PD are initially undefined and do not appear in the PD plot. Nonetheless, samples with lower PD show up very early during the training, which helps us detect shortcuts early. Early detection can consequently help develop intervention schemes that fix the shortcut early. 

\subsection{Prediction Depth $\approx \mathcal{V}\text{-Usable Information}$}
\label{expts_subsec:pd_pvi_rship}

Table-\ref{tab:pd_eq_pvi} measures the influence of spurious features on NIH and KMNIST using PD and PVI metrics. All diseased patients in the ``NIH w/ Spurious feat.'' dataset have a chest drain, whereas all diseased patients in the ``NIH w/o Spurious feat.'' dataset have no chest drain. The set of healthy patients is common for the two datasets. The KMNIST datasets are the same as those used in Section-\ref{subsec:main_expts_toy_medical}. We use VGG16 for KMNIST and DenseNet121 for NIH. Other training details are the same as Section-\ref{subsec:main_expts_toy_medical}. 

\begin{table}[!h]
\caption{Effect of Spurious features on Prediction Depth and the negative conditional $\mathcal{V}\text{-entropy}$ (-$\boldsymbol{H_{\cV_{cnn}}}(Y \mid X)$).
The label marginal distributions are the same with or without the spurious feature, and thus the negative conditional $\mathcal{V}\text{-entropy}$ is proportional to  $\mathcal{V}\text{-information}$.
}
\label{tab:pd_eq_pvi}
\begin{center}
\small
    \begin{tabular}{ccc}
    \hline
    \multicolumn{1}{c}{\bf Dataset}  &\multicolumn{1}{c}{\bf mean PD} &\multicolumn{1}{c}{\bf $-\boldsymbol{H_{\cV_{cnn}}}(Y \mid X)$} \Tstrut{} \Bstrut{}\\
    \hline 
    NIH w/ Spurious feat.     & 53.43 & -0.1171 \Tstrut{}\\
    NIH w/o Spurious feat.    & 75.33 & -0.2321\\
    KMNIST w/ Spurious feat.  & 1.06 & -0.0024 \\
    KMNIST w/o Spurious feat. & 5.25 & -0.0585 \Bstrut{}\\
    \hline
    \end{tabular}
\end{center}
\end{table}


Table-\ref{tab:pd_eq_pvi} shows that datasets with spurious features ($D_s$) have smaller mean PD values than their counterparts without such features ($D_i$). Proposition-1 (see Section-\ref{sec:background}, Appendix-\ref{subsec:proof_prop1}) shows that a sufficient gap between the mean PDs of $D_s$ and $D_i$ causes the $\mathcal{V}$-Information of $D_s$ to be greater than $D_i$. Table-\ref{tab:pd_eq_pvi} confirms this in a medical-imaging dataset with a real chest drain spurious feature, and we see that the mean ``usable information'' increases when there is a spurious feature. This implies that the model learns spurious features as they have more usable information than the core features. We investigate this relationship between PD and $\mathcal{V}$-information in more detail in Appendix-\ref{appdx:pd_pvi_rship}. \citet{swabha_pvi} also show that $\mathcal{V}$-information is positively correlated with test accuracy. This explains the significant change in AUC observed in Fig-\ref{fig:nih_results}D. Proposition 1 bridges the gap between the notions of PD and $\mathcal{V}$-usable information. This connection between $\mathcal{V}$-information and PD indicates that monitoring early training dynamics using PD not only helps detect shortcut learning but also bears insights into the dataset's difficulty (in information-theoretic terms) for a given model class. 



==> sections/old_v1/introduction.tex <==
\textit{Shortcuts} are spurious features that perform well on standard benchmarks but fail to generalize to real-world settings~\citep{geirhos2020shortcut}. Deep neural networks (DNNs) tend to rely on shortcuts even in the presence of \textit{core} features that generalize well, which poses serious problems when deploying them in safety-critical applications such as finance, healthcare, and autonomous driving~\citep{geirhos2020shortcut,luke_tube_in_lung,degrave_covid_shortcut}. Previous works view shortcut learning as a distribution shift problem~\citep{kirichenko2022_last_layer_retraining,wiles2021fine,andrew_beam_structural_characterization,adnan2022monitoring_shortcut_learning}. However, we show that not all spurious correlations are shortcuts. Models suffer from shortcut learning only when the spurious features are much easier to learn than signals that generalize well. We show how monitoring example difficulty metrics like Prediction Depth (PD)~\citep{baldock2021_predictionDepth} can reveal valuable insights into shortcut learning quite early during the training process. Early detection of shortcut learning is helpful as it can help develop intervention schemes to fix the shortcut early. To the best of our knowledge, we are the first to detect shortcut learning by monitoring the training dynamics of the model.

\citet{geirhos2020shortcut} define shortcuts as spurious correlations that exist in standard benchmarks but fail to hold in more challenging test conditions, like real-world settings. The emphasis on shortcuts being synonymous with spurious correlations has led to the widespread adoption of viewing shortcut learning as a distribution shift problem~\citep{andrew_beam_structural_characterization,wiles2021fine,adnan2022monitoring_shortcut_learning,kirichenko2022_last_layer_retraining}. While the distribution shift explains part of the story, we emphasize that what is equally important for shortcut learning is the difficulty of the spurious features themselves (see Fig-\ref{fig:spurious_vs_shortcut}). Previous works like \citet{shah2020pitfalls,scimeca2021shortcut} hint at this. But we take this line of thought further by viewing shortcut learning as a phenomenon that impacts the dataset difficulty, which can be captured by monitoring early training dynamics.

The premises that support our hypothesis are as follows: \textbf{\textit{(P1)}} Shortcuts are only those spurious features that are \textit{``easier''} to learn than the core features (see Fig-\ref{fig:spurious_vs_shortcut}). \textbf{\textit{(P2)}} Initial layers of a DNN tend to learn easy features, whereas the later layers tend to learn the harder ones \citep{zeiler2014visualizing,baldock2021_predictionDepth}. \textbf{\textit{(P3)}} Easy features are learned much earlier than the harder ones during training~\citep{mangalam2019deep,rahaman2019spectral}. Premises~\textbf{\textit{(P1-3)}} lead us to conjecture that: \textit{``Easy features learned by the initial layers of a DNN early during the training are potential shortcuts.''}

We make the following observations. First, when the spurious features are \emph{known}, the paper sheds light on when and if we should be concerned about learning shortcuts. 
We show that a mismatch in the joint distribution of the input, spurious feature, and label between test and training data is insufficient to explain the shortcut learning phenomenon. It also depends on the model's architecture and training dynamics~(section-\ref{subsec:not_all_spurious}). Second, when the spurious feature is \emph{unknown} a priori, but a human user has an intuition about the difficulty of the task in comparison to some reference tasks, the proposed metric can be used to detect shortcut learning patterns during training~(figure-\ref{fig:kmnist_expts}). Third, we empirically show that our hypothesis works well on medical and vision datasets~(sections-\ref{subsec:main_expts_toy_medical},\ref{appdx:vision_expts}), both simulated and real, regardless of the DNN architecture used. We justify this empirical success by theoretically connecting prediction depth with information-theoretic concepts like $\mathcal{V}$-usable information~\citep{swabha_pvi} (sections-\ref{sec:background},\ref{subsec:proof_prop1}). Lastly, our experiments highlight that monitoring only accuracy during training, as is common in machine learning pipelines, is insufficient. In addition, we need to monitor the learning dynamics of the model using suitable instance difficulty metrics to detect shortcut learning (section-\ref{expt:detect_shortcut_early}). This could save time and computational costs and help develop reliable models that do not rely on spurious features.
 
 \begin{figure}[t!]
    \centering
    \centerline{\includegraphics[width=0.85\textwidth, trim = 0cm 3cm 0cm 0cm]{figures/causal_view.pdf}}
    \caption{An illustration of how the causal view of shortcut learning is insufficient. In the causal view, training and testing are different graphical models between input ($x$), output ($y$), and the spurious feature ($s$). If $x$ can predict $s$, and $y$ is not causally related to s on the test data, then $s$ is viewed as a shortcut. (A) The figure shows two scenarios for even-odd classification. Scenario 1 shows a dataset where all even numbers have a spurious composite number (located at the top-left), and odd numbers have a prime number. Scenario 2 shows a dataset where all odd numbers have a spurious white patch. The spurious white patch is an easy feature, so the model uses it as a shortcut. Whereas classifying prime numbers, as shown in scenario 1, is challenging. So the model ignores such spurious features. This shows not all spurious correlations are shortcuts.}
    \label{fig:spurious_vs_shortcut}
\end{figure}
%  trim=left bottom right top











==> sections/old_v1/related_work.tex <==
\paragraph{Not all spurious correlations are shortcuts:} \citet{geirhos2020shortcut} define shortcuts as spurious correlations that exist in standard benchmarks but fail to hold in more challenging test conditions. \citet{wiles2021fine} view shortcut learning as a distribution shift problem where two or more attributes are correlated during training but are independent in the test data. \citet{andrew_beam_structural_characterization} use causal diagrams to explain shortcuts as spurious correlations that hold during training but not during deployment. 
All these papers characterize shortcuts purely as a consequence of distribution shift; methods exist to build models robust to such shifts~\citep{arjovsky2019invariant,krueger2021out,puli2021_nurd}. In contrast, we stress that not all spurious correlations are shortcuts. Rather only those spurious features that are easier than the core features are potential shortcuts (see Fig-\ref{fig:spurious_vs_shortcut}). Previous works like \citet{shah2020pitfalls,scimeca2021shortcut} hint at this by saying that DNNs are biased towards simple solutions, and \citet{too_good_to_be_true_prior} use the ``too-good-to-be-true'' prior to emphasize that simple solutions are unlikely to be valid across contexts. \citet{veitch2021counterfactual} distinguish various model features using tools from causality and stress test the models for counterfactual invariance. 
Other works in natural language inference, visual question answering, and action recognition, also assume that simple solutions could be potential shortcuts~\citep{simple_solutions_are_shortcuts5,simple_solutions_are_shortcuts3,simple_solutions_are_shortcuts2,simple_solutions_are_shortcuts4,simple_solutions_are_shortcuts1}.
We take this line of thought further by viewing shortcuts as simple solutions or, more explicitly, easy features, which affect the early training dynamics of the model. We suggest using suitable example difficulty metrics to measure this effect.

\paragraph{Estimating Example Difficulty:} There are different metrics in the literature for measuring instance-specific difficulty~\citep{agarwal2022_variance_of_grad,hooker2019compressed,lalor2018understanding}. \citet{jiang2020_char_structural} train many models on data subsets of varying sizes to estimate a consistency score that captures the probability of predicting the true label for a particular example. \citet{toneva2018empirical_forgetting} define example difficulty as the minimum number of iterations needed for a particular example to be predicted correctly in all subsequent iterations. \citet{agarwal2022_variance_of_grad} propose a VoG (variance-of-gradients) score which captures example difficulty by averaging the pre-softmax activation gradients across training checkpoints and image pixels. \citet{feldman2020neural} use a statistical viewpoint of measuring example difficulty and develop influence functions to estimate the actual leave-one-out influences for various examples. \citet{swabha_pvi} use an information-theoretic approach to propose a metric called pointwise $\mathcal{V}$-usable information (PVI) to compute example difficulty. \citet{baldock2021_predictionDepth} define prediction depth (PD) as the minimum number of layers required by the DNN to classify a given input and use this to compute instance difficulty. In our experiments, we use the PD metric to provide a proof of concept for our hypothesis.

\paragraph{Monitoring Training Dynamics:} Other works that monitor training dynamics have a significantly different goal than ours. While we monitor training dynamics to detect shortcut learning, \citet{rabanser2022_selective_classification} use neural network training dynamics for selective classification. They use the disagreement between the ground truth label and the intermediate model predictions to reject examples and obtain a favorable accuracy/coverage trade-off. \citet{feng2021phases_of_learning_dynamics} use a statistical physics-based approach to study the training dynamics of stochastic gradient descent (SGD). While they study the effect of mislabeled data on SGD training dynamics, we study the effect of shortcut learning on the early-time learning dynamics of DNNs. \citet{hu2020surprising_simplicity} use the early training dynamics of neural networks to show that a simple linear model can often mimic the learning of a two-layer fully connected neural network. \citet{adnan2022monitoring_shortcut_learning} have a similar goal as ours and use mutual information to monitor shortcut learning. However, computing mutual information is intractable for high-dimensional data, and hence their work is only limited to infinite-width neural networks that offer tractable bounds for this computation. Our work, on the contrary, is more general and holds for different neural network architectures and datasets.


==> sections/old_v2/abstract.tex <==
\emph{Shortcuts} are spurious features that damage the generalization of the Deep Neural Network (DNN) during deployment. This paper aims to better understand shortcut learning through the lens of the learning dynamics of the internal neurons during the training process. We make the following observations: (1) While previous works treat shortcuts as synonymous with spurious correlations, we make a distinction by emphasizing that not all spurious correlations hurt the model generalization. We empirically show that only those spurious features that are ``easier'' than the core features tend to hurt the model generalization. We refer to such spurious features as ``shortcuts''. (2) We build upon this premise and use \emph{instance difficulty} methods (like Prediction Depth~\citep{baldock2021_predictionDepth}) to quantify ``easy'' and to identify this behavior during the training phase. (3) We empirically show that shortcut learning can be detected by observing the learning dynamics of the DNN's \emph{early layers}. In other words, easy features learned by the initial layers of a DNN early during the training tend to hurt model generalization, and are therefore potential shortcuts. We verify our claims on medical and vision datasets, both simulated and real, and justify the empirical success of our hypothesis by showing the theoretical connections between Prediction Depth and information-theoretic concepts like $\mathcal{V}$-usable information~\citep{swabha_pvi}. Lastly, monitoring only accuracy plots during training (as is common in machine learning pipelines) is insufficient to detect shortcut learning patterns, and our experiments therefore highlight the need for monitoring early training dynamics using suitable instance difficulty metrics.

==> sections/old_v2/background.tex <==
 In this section, we formalize the notion of spurious features, shortcuts, and task difficulty. Let $P_{tr}$ and $P_{te}$ be the training and test distributions defined over the random variables $\rmX$ (input), $\rvy$ (label), and $\rvs$ (\emph{latent} spurious feature).


\paragraph{Spurious Feature ($\rvs$):} A latent feature $\rvs$ is called spurious if it is correlated with label $\rvy$ in the training data but not in the test data. Specifically, the joint probability distributions $P_{tr}$ and $P_{te}$ can be factorized as follows.
\begin{equation}
    P_{tr}(\rmX,\rvy,\rvs) = P_{tr}(\rmX|\rvs,\rvy) P_{tr}(\rvs|\rvy)P_{tr}(\rvy) \nonumber
\end{equation}
\begin{equation}
    P_{te}(\rmX,\rvy,\rvs) = P_{tr}(\rmX|\rvs,\rvy) P_{te}(\rvs)P_{tr}(\rvy). \nonumber
\end{equation}
The variable $\rvs$ appears to be related to $\rvy$ but is not. This is shown in Fig-\ref{fig:spurious_vs_shortcut}. We also need a notion of task difficulty. The difficulty of a task depends on the model and data distribution ($\rmX, \rvy$).



\paragraph{Task Difficulty ($\Psi$):}
Let $\Psi^{P}_{\mathcal{M}}(\rmX \rightarrow \rvy)$ indicate the difficulty of predicting $\rmX \rightarrow \rvy$ for a model $\mathcal{M}$, where $\rmX,\rvy \sim P$. Consider a joint distribution $(\rmX,\rvy,\rvt) \sim P$ for two tasks, $\rvt$, and $\rvy$. Then, $\Psi^{P}_{\mathcal{M}}(\rmX \rightarrow \rvy) > \Psi^{P}_{\mathcal{M}}(\rmX \rightarrow \rvt)$ indicates that the task $\rmX \rightarrow \rvy$ is harder than $\rmX \rightarrow \rvt$ for a given model $\mathcal{M}$.


\paragraph{Shortcut:} We define shortcuts as spurious features that hurt model generalization, meaning that the model performs well on $P_{tr}$ but fails to generalize to $P_{te}$. Our empirical findings reveal that a spurious feature damages generalization and acts like a shortcut for model $\mathcal{M}$ iff $\Psi^{P_{tr}}_{\mathcal{M}}(\{\rmX-\rvs\} \rightarrow \rvy) > \Psi^{P_{tr}}_{\mathcal{M}}(\rmX \rightarrow \rvy)$. In other words, removing the spurious feature $\rvs$ from the input $\rmX$ makes it harder for model $\mathcal{M}$ to predict the true label $\rvy$. 

The definitions make it clear that ``shortcut'' is not just related to the dataset alone but is also closely tied to the model and the task. A spurious feature may act like a shortcut for one model and not so for another. E.g., consider input  $X = \{x_1,x_2,…,x_n\}$ that can be viewed as both a vector or a set. Consider two models, $f_1$, which is a permutation-invariant function (like Deep Sets~\citep{deep_sets}), and $f_2$ is a coordinate-sensitive function (e.g., MLP). If the spurious feature is always in $x_1$, it can be a shortcut for $f_2$, but may not be so for $f_1$ because $f_1$ is coordinate agnostic. In fact one can show~\citep{deep_sets} that $f_1 = \rho(\sum_i \phi(x_i))$  for suitable transformations $\phi$ and $\rho$.



We now explain two metrics (Prediction Depth and $\mathcal{V}$-Usable Information) to measure $\Psi^{P}_{\mathcal{M}}$. \citet{baldock2021_predictionDepth} proposed the notion of Prediction Depth (PD) to estimate example difficulty. The PD of input is defined as the minimum number of layers required by the model to classify the input. Our work relies on monitoring early training dynamics using example difficulty metrics, and we use PD estimation for this purpose. The PD metric is also well-suited for our work as it is defined for easy inputs even when the DNN is not fully trained. We use a binary classification setting to explain the concepts used in this section. 

\paragraph{Notion of Prediction Depth:} The PD is defined by building $k$-NN classifiers on the embedding layers of the model. The PD is simply the earliest layer after which all subsequent $k$-NN predictions remain the same (0 or 1):
\begin{equation}
    \text{PD} = \min \argmax_{n} \left[ \prod_{i=n}^{N}f_{knn}(\phi^i) + \prod_{i=n}^{N}(1-f_{knn}(\phi^i)) \right], \nonumber
\end{equation}

$f_{knn}$ is a $k$-NN classifier that outputs 0 or 1 based on a given threshold (see Appendix-\ref{appdx:undefined_PD} for details), $\phi^i$ is the feature embedding for the given input at layer-$i$, and $N$ is the index of the final layer of the model. The lower the PD of input, the easier it is to classify. We also use the notion of undefined PD to work with models that are not fully trained. We treat $k$-NN predictions close to 0.5 (for a binary classification setting) as invalid. If the $k$-NN predictions for the last three layers (for a given input to the model) are invalid, we treat the PD of the input as undefined (see Appendix-\ref{appdx:undefined_PD}). Figure-\ref{fig:pd_plot_explain} illustrates how to read the PD plots used in our experiment.

 \begin{figure*}[ht!]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth, trim = 0cm 6cm 0cm 0cm]{figures/pd_plot_explain.pdf}}
    \caption{Examples of PD plots (for DenseNet-121) at different stages of the training process. The red bar indicates samples with undefined PD, and the dotted vertical line indicates the mean PD of the plot. Notice that the undefined samples (shown in red) slowly accumulate in layer 88 as training progresses. This is because the model needs more time to learn the challenging samples which accumulate at higher prediction depth, i.e., later layers.}
    \label{fig:pd_plot_explain}
\end{figure*}
%  trim=left bottom right top

\paragraph{Notion of $\mathcal{V}$-Usable Information:} The Mutual Information between input and output, $I(X; Y)$, is invariant with respect to lossless encryption of the input, i.e., $I(\tau(X); Y) = I(X; Y)$. Such a definition assumes unbounded computation and is counter-intuitive to define task difficulty as heavy encryption of $X$ does not change the task difficulty. The notion of \textit{``Usable Information''} introduced by~\citet{xu2020_usable_info} assumes bounded computation based on the model family $\mathcal{V}$ under consideration. Usable information is measured under a framework called \textit{predictive $\mathcal{V}$-information}~\citep{xu2020_usable_info}. \citet{swabha_pvi} introduce \textit{pointwise $\mathcal{V}$-information} (PVI) for measuring example difficulty. 
\begin{align} \label{pvi_eq}
    \text{PVI}(x \rightarrow y) = -\log_2g[\phi](y) + \log_2g'[x](y), \\
    \text{s.t.}  \quad g,g' \in \mathcal{V} \nonumber
\end{align}
The function $g$ is trained on $(\phi,y)$ input-label pairs, where $\phi$ is a null input that provides no information about the label $y$. $g'$ is trained on $(x,y)$ pairs from the training data. Lower PVI instances are harder for $\mathcal{V}$ and vice-versa. Since the first term in Eq-\ref{pvi_eq} corresponding to $g$ is independent of the input $x$, we only consider the second term having $g'$ in our experiments. In what follows, we relate the notions of PD and $\mathcal{V}$-usable information. We use $\mathcal{V}_{cnn}$ (of finite depth and width) in our proof as our experiments mainly use CNN architectures. 
\paragraph{Proposition 1:} (Informal) Consider two datasets: $D_s \sim P_{tr}(\rmX,\rvy)$ with spurious features and $D_i \sim P_{te}(\rmX,\rvy)$ without them. For some mild assumptions on PD (see Appendix-\ref{subsec:proof_prop1}), if the mean PD of $D_s$ is less than the mean PD of $D_i$, then the $\cV_{cnn}$-usable-information for $D_s$ is larger than the  $\cV_{cnn}$-usable-information for $D_i$: $\cI_{\cV_{cnn}}^{D_s}(X \rightarrow Y) > \cI_{\cV_{cnn}}^{D_i}(X \rightarrow Y)$. \\

See proof in Appendix-\ref{subsec:proof_prop1}. The proposition intuitively implies that a sufficient gap between the mean PD of spurious and core features can result in spurious features having more $\cV_{cnn}$-usable information than core features. In such a scenario, the model will be more inclined to learn spurious features instead of core ones. This proposition justifies using the PD metric to detect shortcut learning, as demonstrated in the following experiments.

==> sections/old_v2/conclusion.tex <==
We study shortcut learning by monitoring the early training dynamics of deep neural networks (DNNs). We empirically show that not all spurious correlations hurt the DNN's generalization, and only those spurious features that are easier than the core features do. We term such spurious features as ``shortcuts''. \textit{``Potential shortcuts can be found by monitoring the easy features learned by the initial layers of a DNN early during the training.''} We validate this hypothesis on real medical and vision datasets. We show that shortcuts are learned quite early during the training and one can detect shortcut learning by monitoring the early training of DNNs using instance difficulty metrics like Prediction Depth (PD). Further, we show a theoretical connection between PD and $\mathcal{V}$-information to support our empirical results. Datasets with spurious features have more $\mathcal{V}$-information as compared to their counterparts without such features causing the model to learn the shortcut. To conclude, relying only on accuracy plots is insufficient for detecting shortcut learning, and we recommend monitoring the DNN training dynamics using instance difficulty metrics like PD for the early detection of shortcuts.


==> sections/old_v2/experiments.tex <==
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-1.0ex]{0pt}{0pt}}   % = `bottom' strut

We set up four experiments to evaluate our hypothesis. 
\textit{First}, we consider two kinds of datasets, one where the spurious feature is easier than the core feature and another where the spurious feature is harder. We train a classifier on each dataset and observe that the model can learn the easy spurious feature but not the harder one. This experiment demonstrates that not all spurious correlations hurt generalization, but only those spurious features that are easier than the core features are used by the model as shortcuts.
\textit{Second}, we use medical and vision datasets to demonstrate how monitoring the learning dynamics of the initial layers can reveal suspicious shortcut learning activity. We show that an early peak in the PD plot indicates potential shortcuts, and visualization techniques like grad-CAM can provide intuition about the feature used at that layer.
\textit{Third}, we show how shortcuts can often be detected relatively early during training. This is because initial layers which learn the shortcuts converge very early during the training. We observe this by monitoring PD plots across training epochs. In all of our experiments, the shortcut is revealed by the PD plot within two epochs of training.
\textit{Fourth}, we show that datasets with easy spurious features have more ``usable information''~\citep{swabha_pvi} compared to their counterparts without such features. Due to higher usable information, the model requires fewer layers to classify the images with spurious features. We use this experiment to empirically justify Proposition-1 outlined in Appendix-\ref{subsec:proof_prop1}.

\setcounter{figure}{3} 
\setcounter{table}{1} 
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.0\textwidth, trim = 0cm 8cm 0cm 0cm]{figures/domino_fig.pdf}    \label{fig:domino_fig}
\end{figure*}
%  trim=left bottom right top

\subsection{Not all spurious features hurt generalization}
\label{subsec:not_all_spurious}
We use the Dominoes binary classification dataset (formed by concatenating two datasets vertically; see Fig-3) similar to the setup of \citet{kirichenko2022_last_layer_retraining}. The bottom (top) image acts as the core (spurious) feature. Images are of size $64 \times 32$. We construct three pairs of domino datasets such that each pair has both a hard and an easy spurious feature with respect to the common core feature (see Table-1). We use classes \{0,1\} for MNIST and SVHN, \{coat,dress\} for FMNIST,  and \{airplane, automobile\} for CIFAR10. We also include two classes from Kuzushiji-MNIST (or KMNIST) and construct a modification of this dataset called KMNpatch, which has a spurious patch feature (5x5 white patch on the top-left corner) for one of the two classes of KMNIST. The spurious features are perfectly correlated with the target. The order of dataset difficulty based on the mean-PD is as follows: KMNpatch(1.1) $<$ MNIST(2.2) $<$ FMNIST(3.9) $<$ KMNIST(5) $<$ SVHN(5.9) $<$ CIFAR10(6.8). We use a ResNet18 model and measure the test and core-only accuracies. The test accuracy is measured on a held-out dataset sampled from the same distribution. For the core-only accuracy, we blank out the spurious feature (top-half image) by replacing it with zeroes (same as~\citet{kirichenko2022_last_layer_retraining}). The higher the core-only accuracy, the lesser the model's reliance on the spurious feature, and better is the generalization of the model.


% \begin{minipage}{0.4\textwidth}  %------------------for Figure-------------
% \begin{figure}[H]
% \centering
% \includegraphics[width=1\textwidth]{figures/domino_pic.pdf}
% \caption{{\color{magenta}Dominoes Dataset}}\label{fig:domino_pic_label}
% \end{figure}
% \end{minipage}
% \begin{minipage}[HT]{0.6\textwidth}      %------------------for Table-------------
% % \centering
% \begin{table}[H]
% \centering
% %\captionsetup{type=table} %% tell latex to change to table
%     \tiny
%     \begin{tabular}{cccc}
%         \hline 
%         \multicolumn{1}{c}{\bf Dataset}  &\multicolumn{1}{c}{\bf Is spurious} &\multicolumn{1}{c}{\bf Test} &\multicolumn{1}{c}{\bf Core-only} \Tstrut{}\\ 
%         \multicolumn{1}{c}{\bf (Spurious-Core)} &\multicolumn{1}{c}{\bf harder than core?} &\multicolumn{1}{c}{\bf Accuracy} &\multicolumn{1}{c}{\bf Accuracy} \Bstrut{}\\ 
%         \hline 
%         CIF(6.8) - FMN(3.9) & yes & 99.12$\pm$0.27\% & 98.95$\pm$0.30\% \Tstrut{}\\
%         MN(2.2) - FMN(3.9) & no & 99.95$\pm$0.05\% & 50.75$\pm$2.96\% \Bstrut{}\\
%         \hline
%         CIF(6.8) - KMN(5) & yes & 98.91$\pm$0.16\% & 98.30$\pm$1.08\% \Tstrut{}\\
%         MN(2.2) - KMN(5) & no & 99.97$\pm$0.05\% & 50.48$\pm$2.64\% \Bstrut{}\\
%         \hline
%         CIF(6.8) - MN(2.2) & yes & 99.74$\pm$0.07\% & 99.5$\pm$0.66\% \Tstrut{}\\
%         KMNpatch(1.1) - MN(2.2) & no & 99.97$\pm$0.04\% & 68.78$\pm$20.03\% \Bstrut{}\\
%         \hline 
%     \end{tabular}
% \caption{{\color{magenta}Results for the Dominoes experiment averaged across 4-runs. Numbers in bracket show mean-PD (dataset-difficulty). Core-only accuracy indicates the model's reliance on core features. Models achieve high core-only accuracy when spurious features are harder than core features.}}\label{dominoes_expts}
% \end{table}
% \end{minipage} 

Table 1 shows that all datasets achieve a high test accuracy as expected. The core-only accuracy stays high ($>$98\%) for datasets where the spurious feature is harder to learn than the core feature, indicating the model's high reliance on core features. When the spurious feature is easier than the core, the model learns to leverage them, and hence the core-only accuracy drops to nearly random chance ($\sim$50\%). Interestingly, the KMNpatch-MN results have a much higher core-only accuracy ($\sim$69\%) and a more significant standard deviation. We explain this phenomenon in Appendix-\ref{appdx:pd_perspective_feature_learning}. This experiment demonstrates that only those spurious features that are easier than the core features hurt the generalization of the model harder than the core feature fails to act as a shortcut that the model can leverage to ``cheat''.

\subsection{Monitoring Initial Layers Can Reveal Suspicious Shortcut Learning Activity}
%  Initial layers hold valuable information about shortcuts!
\label{subsec:main_expts_toy_medical}

\paragraph{Synthetic Spurious Feature on Toy Dataset:} To provide a proof of concept, we demonstrate our method on the Kuzushiji-MNIST (KMNIST)~\citep{kmnist} dataset comprising Japanese Hiragana characters. The dataset has ten classes and images of size $28\times28$, similar to MNIST. We insert a white patch (spurious feature) at a particular location for each of the ten classes. The location of the patch is class-specific. We train two VGG16 models, one on the KMNIST with a patch shortcut ($\mathcal{M}_{sh}$) and another on the original KMNIST without the patch ($\mathcal{M}_{orig}$). 

\begin{figure*}[!t]
    \centering
    \centerline{\includegraphics[width=1\textwidth, trim = 0cm 2cm 0cm 0cm]{figures/kmnist_expts.pdf}}
    \caption{Top row shows three reference datasets and their corresponding prediction depth (PD) plots. The datasets are ordered based on their difficulty (measured using mean PD shown by dotted vertical lines): KMN w/ sh.(1.1) $<$ MNIST(2.2) $<$ FMNIST(3.9) $<$ KMN w/o sh.(5) $<$ SVHN(5.9) $<$ CIFAR10(6.8). The bottom row shows the effect of the spurious white patch on the KMNIST dataset. The yellow region on the axis indicates the expected difficulty of classifying KMNIST. While the original KMNIST lies in the yellow region, the spurious feature significantly reduces the task difficulty as it is used by the model as a shortcut. The Grad-CAM shows that the model focuses on the spurious patch.}
    \label{fig:kmnist_expts}
\end{figure*}
%  trim=left bottom right top

Fig-\ref{fig:kmnist_expts} shows the prediction depth (PD) plots for this experiment. The vertical dashed lines show the mean PD for each plot. Fig-\ref{fig:kmnist_expts}D shows that KMNIST with patch has a much lower mean PD than all the other datasets, and the PD plot is also highly skewed towards the initial layers. This suspicious behavior is because the white patch is a very easy feature, and hence the model only needs a single layer to detect it. The Grad-CAM maps for layer-1 confirm this by showing that $\mathcal{M}_{sh}$ focuses mainly on the patch (see Fig-\ref{fig:kmnist_expts}D), and hence the test accuracy on the original KMNIST images is very low ($\sim$8\%). The PD plot for $\mathcal{M}_{orig}$ (see Fig-\ref{fig:kmnist_expts}E) is not as skewed toward lower depth as the plot for $\mathcal{M}_{sh}$. This is expected as $\mathcal{M}_{orig}$ is not looking at the spurious patch and therefore utilizes more layers to make the prediction. The mean PD for $\mathcal{M}_{orig}$ suggests that the original KMNIST is harder than Fashion-MNIST but easier than CIFAR10. $\mathcal{M}_{orig}$ also achieves a higher test accuracy ($\sim$98\%). 

This experiment demonstrates how models that learn spurious features ($\mathcal{M}_{sh}$) exhibit PD plots that are suspiciously skewed towards the initial layers. The skewed PD plot should raise concerns, and visualization techniques like Grad-CAM can aid our intuition about what spurious feature the model may be utilizing at any given layer. 

\paragraph{Semi-Synthetic Spurious Features on Medical Datasets:} \label{sec:semi_synth_expts} We follow the procedure by \citet{degrave_covid_shortcut} to create the ChestX-ray14/GitHub-COVID dataset. This dataset comprises Covid19 positive images from Github Covid repositories and negative images from ChestX-ray14 dataset~\citep{wang_chestxray14_dataset}. In addition, we also create the Chex-MIMIC dataset following the procedure by \citet{puli2021_nurd}. This dataset comprises 90\% images of Pneumonia from Chexpert~\citep{chexpert_dataset} and 90\% healthy images from MIMIC-CXR~\citep{mimic_cxr_dataset}. We train two DenseNet121 models,  $\mathcal{M}_{covid}$ on the ChestX-ray14/GitHub-COVID dataset, and $\mathcal{M}_{chex}$ on the Chex-MIMIC dataset. We use DenseNet121, a common and standard architecture for medical image analysis. Images are resized to $512\times512$. 

\begin{figure}[htbp!]
    \centering
    \centerline{\includegraphics[width=0.85\textwidth, trim = 0cm 6cm 0cm 0cm]{figures/semi_synthetic_medical_shortcut.pdf}}
    \caption{PD plots for two DenseNet-121 models trained on Chex-MIMIC and ChestX-ray14/GitHub-COVID datasets are shown in the figure, along with their corresponding Grad-CAM visualizations. Both PD plots exhibit a very high peak in the initial layers (1 to 4), indicating that the models use very easy features to make the predictions.
    }
    \label{fig:semi_synthetic_medical_shortcut}
\end{figure}
%  trim=left bottom right top

Fig-\ref{fig:semi_synthetic_medical_shortcut} shows the PD plots for $\mathcal{M}_{chex}$ and $\mathcal{M}_{covid}$. Both the plots are highly skewed towards initial layers, similar to the KMNIST with spurious patch in Fig-\ref{fig:kmnist_expts}D. This again indicates that the models are using very easy features to make the predictions, which is concerning as the two tasks (pneumonia and covid19 detection) are hard tasks even for humans. Examining the Grad-CAM maps at layer-4 reveals that these models focus on spurious features outside the lung region, which are irrelevant because both diseases are known to affect mainly the lungs. The reason for this suspicious behavior is that, in both these datasets, the healthy and diseased samples have been acquired from two different sources.
This creates a spurious feature because source-specific attributes or tokens are predictive of the disease and can be easily learned, as pointed out by \citet{degrave_covid_shortcut}.


\paragraph{Real Spurious Feature on Medical Dataset:} For this experiment, we use the NIH dataset~\citep{nih_dataset} which has the popular chest drain spurious feature (for Pneumothorax detection)~\citep{luke_tube_in_lung}. Chest drains are used to treat positive Pneumothorax cases. Therefore, the presence of a chest drain in the lung is positively correlated with the presence of Pneumothorax and can be used by the deep learning model~\citep{luke_tube_in_lung}. Appendix-\ref{subsec:nih_chest_drains} outlines the procedure we use to obtain chest drain annotations for the NIH dataset. We train a DenseNet121 model ($\mathcal{M}_{nih}$) for Pneumothorax detection on NIH images of size $128\times128$. 

\begin{figure*}[h!]
    \centering
    \centerline{\includegraphics[width=0.9\textwidth, trim = 0cm 7cm 3cm 0cm]{figures/nih_results2.pdf}}
    \caption{Shortcut learning on NIH dataset. (A) PD plot for DenseNet-121 trained on NIH shows prominent peaks in the initial layers. (B, C) Grad-CAM reveals that the initial layers use irrelevant artifacts and chest drains as shortcuts for classification. (D) The chest drain spurious feature affects the AUC performance of the model. The X-axis (Y-axis) shows the false positive (true positive) rate.}
    \label{fig:nih_results}
\end{figure*}
%  trim=left bottom right top

Fig-\ref{fig:nih_results}A shows the PD plot for $\mathcal{M}_{nih}$. We observe that the distribution is not as skewed as the plots in the previous experiments. This is because all the images come from a single dataset (NIH). However, we do see suspicious peaks at the initial layers. Pneumothorax classification is challenging even for radiologists; hence, peaks at the initial layers raise suspicion. The Grad-CAM maps in Figs-\ref{fig:nih_results}B \& \ref{fig:nih_results}C reveal that the initial layers look at irrelevant artifacts and chest drains in the image. This provides evidence for shortcut learning happening in the initial layers. Fig-\ref{fig:nih_results}D shows that the AUC performance is 0.94 when the diseased patients have a chest drain and 0.74 when they don't. In both cases, the set of healthy patients remains the same. This observation is consistent with the findings of \citet{luke_tube_in_lung} and indicates that the model looks at chest drains to classify positive Pneumothorax cases. 

The above experiments demonstrate how a peak located in the initial layers of the PD plot should raise suspicion, especially when the classification task is challenging. Visualization techniques like Grad-CAM can further aid our intuition and help identify the shortcuts being learned by the model. This approach works well even for realistic scenarios and challenging spurious features (like chest drain for Pneumothorax classification), as shown above. Appendix-\ref{appdx:vision_expts} includes additional results on vision datasets.

\subsection{Detecting Shortcuts Early}
\label{expt:detect_shortcut_early}

Fig-\ref{fig:pd_evolution_nih} shows the evolution of the PD plot across epochs for $\mathcal{M}_{nih}$ (which is the model used in Fig-\ref{fig:nih_results}). This visualization helps us observe the training dynamics of the various layers. The red bar in the PD plots shows the samples with undefined prediction depths. 

\begin{figure*}[t!]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth, trim = 0cm 4cm 0cm 0cm]{figures/nih_evolution_pd_plots.pdf}}
    \caption{Evolution of PD plot across epochs shows the training dynamics of the DNN on the NIH dataset. The initial peaks (layers-4\&40) are relatively stable throughout training, whereas the later peaks (layer-88) change with time. The initial layers learn the easy spurious features, which can be detected early during the training. Samples with undefined PD (shown in red) take more time to converge and eventually accumulate in the later layers (layer 88 in this case).}
    \label{fig:pd_evolution_nih}
\end{figure*}
%  trim=left bottom right top

These plots reveal several useful insights into the learning dynamics of the model. Firstly, we see three prominent peaks in epoch-1 at layers-4,40,88 (see Fig-\ref{fig:pd_evolution_nih}A). The magnitude of the initial peaks (like layers-4\&40) remains nearly constant throughout the training. These peaks correspond to spurious features being used by the model, as discussed in the previous section. This indicates that shortcuts can often be identified early (epoch-1 in this case). Fig-\ref{fig:epoch_2_pd_plot} shows the PD plots at epoch-2 for other datasets with spurious features. It is clear from Fig-\ref{fig:epoch_2_pd_plot} that the suspiciously high peak at the initial layer is visible in the \textit{second epoch} itself. The Grad-CAM maps reveal that this layer looks at irrelevant artifacts in the dataset. This behavior is seen in all datasets shown in Fig-\ref{fig:epoch_2_pd_plot}. 

\begin{figure*}[h!]
    \centering
    \centerline{\includegraphics[width=1.0\textwidth, trim = 0cm 9cm 0cm 0cm]{figures/epoch_2_pd_plot.pdf}}
    \caption{Epoch-2 PD plots for various datasets with spurious features. The high spurious peak in the initial layer is visible in all the datasets indicating that shortcuts can be detected early during the training.}
    \label{fig:epoch_2_pd_plot}
\end{figure*}
%  trim=left bottom right top

Secondly, we also see that accuracy or AUC plots do not reveal shortcut learning patterns. We need to monitor the training dynamics using suitable metrics (like PD) to detect this behavior. Thirdly, the red peak (undefined samples) decreases in magnitude with time, and we see a proportional increase in the layer-88 peak. This corroborates well with the observation that later layers take more time to converge~\citep{rahaman2019spectral,mangalam2019deep,zeiler2014visualizing}. Therefore, samples with higher PD are initially undefined and do not appear in the PD plot. Nonetheless, samples with lower PD show up very early during the training, which helps us detect shortcuts early. Early detection can consequently help develop intervention schemes that fix the shortcut early. 

\subsection{Prediction Depth $\approx \mathcal{V}\text{-Usable Information}$}
\label{expts_subsec:pd_pvi_rship}

Table-\ref{tab:pd_eq_pvi} measures the influence of spurious features on NIH and KMNIST using PD and PVI metrics. All diseased patients in the ``NIH w/ Spurious feat.'' dataset have a chest drain, whereas all diseased patients in the ``NIH w/o Spurious feat.'' dataset have no chest drain. The set of healthy patients is common for the two datasets. The KMNIST datasets are the same as those used in Section-\ref{subsec:main_expts_toy_medical}. We use VGG16 for KMNIST and DenseNet121 for NIH. Other training details are the same as Section-\ref{subsec:main_expts_toy_medical}. 

\begin{table}[!h]
\caption{Effect of Spurious features on Prediction Depth and the negative conditional $\mathcal{V}\text{-entropy}$ (-$\boldsymbol{H_{\cV_{cnn}}}(Y \mid X)$).
The label marginal distributions are the same with or without the spurious feature, and thus the negative conditional $\mathcal{V}\text{-entropy}$ is proportional to  $\mathcal{V}\text{-information}$.
}
\label{tab:pd_eq_pvi}
\begin{center}
\small
    \begin{tabular}{ccc}
    \hline
    \multicolumn{1}{c}{\bf Dataset}  &\multicolumn{1}{c}{\bf mean PD} &\multicolumn{1}{c}{\bf $-\boldsymbol{H_{\cV_{cnn}}}(Y \mid X)$} \Tstrut{} \Bstrut{}\\
    \hline 
    NIH w/ Spurious feat.     & 53.43 & -0.1171 \Tstrut{}\\
    NIH w/o Spurious feat.    & 75.33 & -0.2321\\
    KMNIST w/ Spurious feat.  & 1.06 & -0.0024 \\
    KMNIST w/o Spurious feat. & 5.25 & -0.0585 \Bstrut{}\\
    \hline
    \end{tabular}
\end{center}
\end{table}


Table-\ref{tab:pd_eq_pvi} shows that datasets with spurious features ($D_s$) have smaller mean PD values than their counterparts without such features ($D_i$). Proposition-1 (see Section-\ref{sec:background}, Appendix-\ref{subsec:proof_prop1}) shows that a sufficient gap between the mean PDs of $D_s$ and $D_i$ causes the $\mathcal{V}$-Information of $D_s$ to be greater than $D_i$. Table-\ref{tab:pd_eq_pvi} confirms this in a medical-imaging dataset with a real chest drain spurious feature, and we see that the mean ``usable information'' increases when there is a spurious feature. This implies that the model learns spurious features as they have more usable information than the core features. We investigate this relationship between PD and $\mathcal{V}$-information in more detail in Appendix-\ref{appdx:pd_pvi_rship}. \citet{swabha_pvi} also show that $\mathcal{V}$-information is positively correlated with test accuracy. This explains the significant change in AUC observed in Fig-\ref{fig:nih_results}D. Proposition 1 bridges the gap between the notions of PD and $\mathcal{V}$-usable information. This connection between $\mathcal{V}$-information and PD indicates that monitoring early training dynamics using PD not only helps detect shortcut learning but also bears insights into the dataset's difficulty (in information-theoretic terms) for a given model class. 



==> sections/old_v2/introduction.tex <==
Deep neural networks (DNNs) tend to rely on spurious features even in the presence of \textit{core} features that generalize well, which poses serious problems when deploying them in safety-critical applications such as finance, healthcare, and autonomous driving~\citep{geirhos2020shortcut,luke_tube_in_lung,degrave_covid_shortcut}. A feature is termed spurious if it is correlated with the label during training but is irrelevant to the learning problem~\citep{saab2022reducing,izmailov2022feature}. While previous works use a distribution shift approach to explain this phenomenon~\citep{kirichenko2022_last_layer_retraining,wiles2021fine,andrew_beam_structural_characterization,adnan2022monitoring_shortcut_learning}, we emphasize upon the learnability and difficulty of spurious features to show that not all spurious features hurt generalization. We empirically find that only those spurious features that are ``easier'' than the core features tend to hurt generalization. We refer to such spurious features as ``shortcuts''. We show how monitoring instance difficulty metrics like Prediction Depth (PD)~\citep{baldock2021_predictionDepth} can reveal valuable insights into shortcut learning quite early during the training process. Early detection of shortcut learning is helpful as it can help develop intervention schemes to fix the shortcut early. To the best of our knowledge, we are the first to use model training dynamics to detect shortcut learning.

The premises that support our hypothesis are as follows: \textbf{\textit{(P1)}} Spurious features hurt model generalization if they are \textit{``easier''} to learn than the core features (see Fig-\ref{fig:spurious_vs_shortcut}). \textbf{\textit{(P2)}} Initial layers of a DNN tend to learn easy features, whereas the later layers tend to learn the harder ones \citep{zeiler2014visualizing,baldock2021_predictionDepth}. \textbf{\textit{(P3)}} Easy features are learned much earlier than the harder ones during training~\citep{mangalam2019deep,rahaman2019spectral}. Premises~\textbf{\textit{(P1-3)}} lead us to conjecture that: \textit{``Easy features learned by the initial layers of a DNN early during the training are potential shortcuts.''}

We make the following observations. First, we show that not all spurious correlations hurt generalization, and only those that are easier to learn than the core features do. Second, we empirically show that our hypothesis works well on medical and vision datasets~(sections-\ref{subsec:main_expts_toy_medical},\ref{appdx:vision_expts}), both simulated and real, regardless of the DNN architecture used. We justify this empirical success by theoretically connecting prediction depth with information-theoretic concepts like $\mathcal{V}$-usable information~\citep{swabha_pvi} (sections-\ref{sec:background},\ref{subsec:proof_prop1}). Lastly, our experiments highlight that monitoring only accuracy during training, as is common in machine learning pipelines, is insufficient to detect shortcut learning. We need to monitor the learning dynamics of the model using suitable instance difficulty metrics to detect this phenomenon (section-\ref{expt:detect_shortcut_early}). This will not only save time and computational costs, but also help develop reliable models that do not rely on spurious features.
 
 \begin{figure}[t!]
    \centering
    \centerline{\includegraphics[width=0.85\textwidth, trim = 0cm 5.5cm 0cm 3cm]{figures/causal_view.pdf}}
    \caption{An illustration of how the distribution shift viewpoint cannot distinguish between shortcuts and other spurious features. This viewpoint suggests that training and testing are different graphical models between input ($x$), output ($y$), and the spurious feature ($s$). If $x$ can predict $s$, and $y$ is not correlated to s on the test data, then $s$ is viewed as a spurious feature. (A) The figure shows two scenarios for even-odd classification. Scenario 1 shows a dataset where all even numbers have a spurious composite number (located at the top-left), and odd numbers have a prime number. Scenario 2 shows a dataset where all odd numbers have a spurious white patch. The spurious white patch is an easy feature, so the model uses it as a shortcut. Whereas classifying prime numbers, as shown in scenario 1, is challenging. So the model ignores such spurious features. This shows not all spurious correlations hurt model generalization.}
    \label{fig:spurious_vs_shortcut}
\end{figure}
%  trim=left bottom right top











==> sections/old_v2/related_work.tex <==
\paragraph{Not all spurious correlations hurt generalization:} \citet{geirhos2020shortcut} define spurious features as features that exist in standard benchmarks but fail to hold in more challenging test conditions. \citet{wiles2021fine} view spurious correlations as a distribution shift problem where two or more attributes are correlated during training but are independent in the test data. \citet{andrew_beam_structural_characterization} use causal diagrams to explain spurious correlations as features that are correlated with the label during training but not during deployment. 
All these papers characterize spurious correlations purely as a consequence of distribution shift; methods exist to build models robust to such shifts~\citep{arjovsky2019invariant,krueger2021out,puli2021_nurd}. The distribution shift viewpoint cannot distinguish between shortcuts vs other spurious features. In contrast, we stress the learnability and difficulty of spurious features, which helps us identify spurious features that hurt generalization by acting as shortcuts (see Fig-\ref{fig:spurious_vs_shortcut}). Previous works like \citet{shah2020pitfalls,scimeca2021shortcut} hint at this by saying that DNNs are biased towards simple solutions, and \citet{too_good_to_be_true_prior} use the ``too-good-to-be-true'' prior to emphasize that simple solutions are unlikely to be valid across contexts. \citet{veitch2021counterfactual} distinguish various model features using tools from causality and stress test the models for counterfactual invariance. 
Other works in natural language inference, visual question answering, and action recognition, also assume that simple solutions could be potential shortcuts~\citep{simple_solutions_are_shortcuts5,simple_solutions_are_shortcuts3,simple_solutions_are_shortcuts2,simple_solutions_are_shortcuts4,simple_solutions_are_shortcuts1}.
We take this line of thought further by hypothesizing that simple solutions or, more explicitly, easy features, which affect the early training dynamics of the model can hurt model generalization. We suggest using suitable instance difficulty metrics to identify such shortcuts.

\paragraph{Estimating Example Difficulty:} There are different metrics in the literature for measuring instance-specific difficulty~\citep{agarwal2022_variance_of_grad,hooker2019compressed,lalor2018understanding}. \citet{jiang2020_char_structural} train many models on data subsets of varying sizes to estimate a consistency score that captures the probability of predicting the true label for a particular example. \citet{toneva2018empirical_forgetting} define example difficulty as the minimum number of iterations needed for a particular example to be predicted correctly in all subsequent iterations. \citet{agarwal2022_variance_of_grad} propose a VoG (variance-of-gradients) score which captures example difficulty by averaging the pre-softmax activation gradients across training checkpoints and image pixels. \citet{feldman2020neural} use a statistical viewpoint of measuring example difficulty and develop influence functions to estimate the actual leave-one-out influences for various examples. \citet{swabha_pvi} use an information-theoretic approach to propose a metric called pointwise $\mathcal{V}$-usable information (PVI) to compute example difficulty. \citet{baldock2021_predictionDepth} define prediction depth (PD) as the minimum number of layers required by the DNN to classify a given input and use this to compute instance difficulty. In our experiments, we use the PD metric to provide a proof of concept for our hypothesis.

\paragraph{Monitoring Training Dynamics:} Other works that monitor training dynamics have a significantly different goal than ours. While we monitor training dynamics to detect shortcut learning, \citet{rabanser2022_selective_classification} use neural network training dynamics for selective classification. They use the disagreement between the ground truth label and the intermediate model predictions to reject examples and obtain a favorable accuracy/coverage trade-off. \citet{feng2021phases_of_learning_dynamics} use a statistical physics-based approach to study the training dynamics of stochastic gradient descent (SGD). While they study the effect of mislabeled data on SGD training dynamics, we study the effect of shortcut learning on the early-time learning dynamics of DNNs. \citet{hu2020surprising_simplicity} use the early training dynamics of neural networks to show that a simple linear model can often mimic the learning of a two-layer fully connected neural network. \citet{adnan2022monitoring_shortcut_learning} have a similar goal as ours and use mutual information to monitor shortcut learning. However, computing mutual information is intractable for high-dimensional data, and hence their work is only limited to infinite-width neural networks that offer tractable bounds for this computation. Our work, on the contrary, is more general and holds for different neural network architectures and datasets.

